PalmBench: A Comprehensive Benchmark of Compressed Large Language Models on Mobile Platforms

Deploying large language models (LLMs) locally on mobile devices is advantageous in scenarios where transmitting data to remote cloud servers is either undesirable due to privacy concerns or impractical due to network connection. Recent advancements (MLC, 2023a; Gerganov, 2023) have facilitated the local deployment of LLMs. However, local deployment also presents challenges, particularly in balancing quality (generative performance), latency, and throughput within the hardware constraints of mobile devices. In this paper, we introduce our lightweight, all-in-one automated benchmarking framework that allows users to evaluate LLMs on mobile devices. We provide a comprehensive benchmark of various popular LLMs with different quantization configurations (both weights and activations) across multiple mobile platforms with varying hardware capabilities. Unlike traditional benchmarks that assess full-scale models on high-end GPU clusters, we focus on evaluating resource efficiency (memory and power consumption) and harmful output for compressed models on mobile devices. Our key observations include i) differences in energy efficiency and throughput across mobile platforms; ii) the impact of quantization on memory usage, GPU execution time, and power consumption; and iii) accuracy and performance degradation of quantized models compared to their non-quantized counterparts; and iv) the frequency of hallucinations and toxic content generated by compressed LLMs on mobile devices.

==> decision.tex <==
Based on our experimental observations, we propose deployment strategies for on-device LLMs, outlining a decision model along three dimensions to guide mobile deployment.
%
In utilizing the MLC framework to deploy a pre-trained model, one can adjust the \textbf{model architecture}, \textbf{quantization scheme}, and \textbf{model size}. These adjustments strike a balance between performance and efficiency, representing the three key dimensions of our decision model.
%
Each dimension corresponds to distinct user needs. For instance, some users are not sensitive to latency and don't mind waiting longer for a more accurate response. Others are conscious of their phone's battery consumption and would prefer the LLM not to drain too much power. Furthermore, some users manage work-related tasks on their mobile devices and would not appreciate the LLM chatbot occupying the device's resources.
%

\iffalse
\begin{algorithm}
        \caption{Mobile LLM Deployment Strategy}
        \label{alg:decision}
        \begin{algorithmic}[1] 
            \Function {"Decision Model"}{}
                %if
                \If {"Device's RAM is less than 4GB"}  "RadPajama-1v-3B-q4f16"  
                \ElsIf {"Time Sensitive"}   "RadPajama-1v-3B-q4f16"       
                \ElsIf {"Energy Efficiency"}  %"text"  
                    \If {"More Accuracy?"} "RadPajama-1v-7B-q4f16"
                    \Else "RadPajama-1v-3B-q4f16" \EndIf%\State 
                \ElsIf {"Reasoning, Math and Coding?"} "Llama-2-13B-q4f16"
                \Else
                     \If {"RAM is more than 8GB?"} "Llama-2-7B-q4f16"
                     \Else "Llama-2-7B-q3f16" \EndIf%\State 
                \EndIf\State                   
                \Return $Result$
            \EndFunction
        \end{algorithmic}
    \end{algorithm}
    \fi

%We structured this decision model in pseudocode~\ref{alg:decision}. 
%
%Larger models demand increased resources but can improve performance and provide more precise answers, while smaller models are more efficient yet may sacrifice accuracy. 
%An appropriate tradeoff should be made considering the target platform's capabilities and user requirements. 
%
As illustrated in Figure~\ref{fig:mtscores}, Llama-2-7B outperforms in delivering more accurate responses, albeit at the expense of longer processing times and increased resource consumption over RedPajama-1v-3B and RedPajama-1v-7B. This makes Llama-2-7B suitable for users who care more about answer precision over response time and have a greater tolerance for latency.
%

For individuals using devices with limited resources, especially those with less than 4GB of memory, RedPajama-1v-3B with 4-bit quantization is a preferable option. The 3-bit quantization scheme q3f16, though offering slight savings in resource usage, latency, and power consumption, falls short of delivering a satisfactory user experience. 
%Conversely, while the 8-bit quantization consumes more resources than the 4-bit scheme q4f16, it doesn't yield improved MTBench scores. 
4-bit quantization q4f16 should be the best option to strike the tradeoff among resource, latency, energy efficiency, and precision on mobile devices.
%
On the other hand, Vicuna-1v-7B underperforms regarding resource efficiency and MT-Bench scores across all three evaluated models, leading us to exclude Vicuna from our deployment strategy.
%
As shown in Sections~\ref{ssec:quan} and Section~\ref{ssec:size}, optimized deployment strategies can improve memory efficiency by up to 19.1\% and boost scores by 34\% on MTBench for on-device LLMs. Appropriate configuration and sizing can yield substantial resource savings and accuracy gains.


Additionally, the evaluation highlights substantial platform differences as depicted in Figure~\ref{fig:eval_platforms}. iOS exhibits lower latency and higher energy efficiency while maintaining greater throughput compared to other mobile operating systems.
%
%
In our experiments, we noted a consistent reliance on GPUs across all platforms for model inference. To enhance efficiency, developers can leverage the full capacity of hardware resources. For instance, MLC has incorporated support for Qualcomm Snapdragon's Hexagon DSP for inference, offering an alternative to shift some tasks from an overburdened GPU to the DSP.
%
Additionally, our observations indicated that the NPU on Apple's A14 consistently showed 0\% utilization, suggesting no tasks were executed on it. Given that the iPhone's GPU usage nears 100\% during LLM chatbot operations, iOS developers might consider offloading model inference tasks to the NPU.


 

==> discuss.tex <==
Our thoroughly benchmarking for mobile LLMs execution yielded several key observations, not limited to resource usage and energy efficiency, but also some potential

\subsection{Efficiency}
Apple's iPhones offer significantly high throughput

==> eval.tex <==

In this section, we conduct experimental evaluations of LLMs on mobile devices using the methodology outlined in Section~\ref{sec:method}. Specifically, we perform experiments across three sets: 1) profiling resource usage and user experience with simple conversational queries, 2) evaluating mobile devices on complex dialog tasks using the MTBench benchmark, and 3) evaluating the impact of model size and quantization parameters. 
%
Based on observations from these experiments, we develop a decision model to guide developers and researchers in selecting appropriate models and compiler configurations optimized for on-device inference, as illustrated in Section~\ref{sec:deploy}. 
%
Our methodology provides data-driven deployment insights tailored to resource-constrained platforms.
%Our mobile-centric methodology and decision model aim to provide data-driven insights and recommendations for maximizing efficiency and user experience when deploying LLMs on resource-constrained mobile platforms.

%In this section, we perform three experiment sets to evaluate LLM on mobile devices, demonstrating how our methodology described in Section~\ref{sec:method} the formulation of efficient deployment strategies optimized for mobile platforms. Based on the observations, e develop a decision model that assists developers and
%researchers in selecting the appropriate model and compiler parameters.
%
%The MLC LLM repository~\cite{MLC_repo} offers sample mobile applications (iOS, Android) and a command line interface (CLI) for Linux systems, aiding us in constructing our benchmarking utilities.

%\vspace{-1ex}

\vspace{-2.5ex}
\subsection{Platforms}
\vspace{-2ex}

%\pan{Aside from speed, and power consumption of quantized models, we also need to run LLM benchmarks (or find existing benchmarks) such as MMLU to understand the performance-speed/energy tradeoff.}
%\yilong{MTBench is better. Because it has pre-defined question sets and scored by GPT4.}

MLC LLM framework supports the platforms of IOS, Android, and Linux.
%
The mobile platform ecosystem is overly fragmented.
%
The platform evaluation mainly focuses on resource usage, latency, and power consumption of LLM applications across different mobile platforms~(e.g., Android, iOS, and embedded systems) by \textbf{Simple Q\&A} test set.
%
We create the \textbf{Simple Q\&A} test set to emulate daily lightweight usage containing straightforward questions without definitive answers, such as greetings, weather inquiries, letter writing, and trip planning. While not evaluating model performance, the \textbf{Simple Q\&A} tests enabled analysis of resource utilization and user experience when posing conversational queries without pre-defined responses.
%
Figure~\ref{fig:eval_platforms} shows the results of resource usage (CPU, GPU, and Memory) while testing \textbf{Simple Q\&A}. Besides the resources, we also evaluated the latency~(ms), throughput~(tok/s), and power consumption in Figure~\ref{fig:latency_thru_power_platforms}. 
%
Not surprisingly, we observe that during LLM inference, the GPU experiences the highest usage, with memory following closely as the second-most utilized component. In comparison, the CPU's utilization is more subdued since LLM inference predominantly leverages the GPU and memory.
%
Additionally, the iPhone 12 Pro exhibited lower resource utilization than other test platforms, indicating the potential for optimization and efficiency of LLM deployment.
%
All tested devices have a high GPU utilization above 80\%, with LLaMa-2-7B and Vicuna-7B saturating the GPU over 90\%. Comparatively, RedPajama-3B demonstrated relatively lower resource usage and faster running speed, indicating it is less resource-intensive and more efficient on mobile platforms in \textbf{Simple Q\&A} task.

\begin{figure}[ht]
\vspace{-2ex}
\setlength\abovecaptionskip{0pt}
\subfigure[LLaMa-2]{
\includegraphics[width=0.32\textwidth]{figures/eval/usagellama.pdf}
\label{fig:usellama}
}
\hspace{-1.5ex}
\subfigure[RedPajama]{
\centering
\includegraphics[width=0.32\textwidth]{figures/eval/usagered.pdf}
\label{fig:usered}
}
\hspace{-1.5ex}
\subfigure[Vicuna]{
\centering
\includegraphics[width=0.32\textwidth]{figures/eval/usagevicuna.pdf}
\label{fig:usevicuna}
}
%\hfill
%\subfigure[Power Consumption]{
%\centering
%\includegraphics[width=0.45\textwidth]{figures/eval/powerplatforms.pdf}
%\label{fig:usevicuna}
%}
%\vspace{-1.5ex}
\caption{Resources utilization (CPU, GPU, and Memory) of different platforms (IP12: iPhone 12 Pro, Pixel 4, S22U: S22 Ultra, and Pi: Orange Pi) and testing models (Llama-2-7B, RedPajama-v1-3B and Vicuna-v1-7B) on a `Simple Q\&A' Task.}
\label{fig:eval_platforms}
\vspace{-.5ex}
\end{figure}

We also evaluated the latency, throughput, and power consumption of various models on these platforms. The metrics for evaluating latency and throughput are \textbf{generation latency} and \textbf{generation throughput.} 
%
Latency is the time consumed to generate an answer, while throughput is defined as the number of generated tokens divided by the sum of \textit{prefill time} and \textit{decoding time}. 
%
We evaluated latency by measuring the interval between clicking the `send' button and the answer generated.


\begin{figure}[ht]
\vspace{-2ex}
\setlength\abovecaptionskip{0pt}
\subfigure[Latency]{
\includegraphics[width=0.32\textwidth]{figures/eval/latencyplatforms.pdf}
\label{fig:latency_platform}
}
\hspace{-1.5ex}
\subfigure[Throughput]{
\centering
\includegraphics[width=0.32\textwidth]{figures/eval/throughputplatforms.pdf}
\label{fig:thru_platform}
}
\hspace{-1.5ex}
\subfigure[Power Consumption]{
\centering
\includegraphics[width=0.32\textwidth]{figures/eval/powerplatforms.pdf}
\label{fig:power_platform}
}
%\vspace{-1.5ex}
\caption{Comparison of latency (s), throughput (Tok/s), and power consumption (mA) of three models (Llama-2-7B, RedPajama-v1-3B and Vicuna-v1-7B) on different mobile platforms (IP12-iPhone 12, Pixel 4, S22U-S22 Ultra and Pi-Orange Pi).}
\label{fig: latency_thru_power_platforms}
\vspace{-.5ex}
\end{figure}

As depicted in Figure~\ref{fig: latency_thru_power_platforms}, evaluation results clearly demonstrate
the iPhone 12 Pro's advantages, consuming low current and lower latency while significantly surpassing the throughput of other platforms.


\vspace{-2ex}
\subsection{Multi-Turn Questions} \label{ssec:mtbench}
\vspace{-1.5ex}
%MTBench utilizes a predefined multi-turn question set to evaluate a chat model's conversational and instruction-following capabilities across turns. The model responses are scored by GPT-4.
MT-bench~\cite{MTBenchArena_2023} employs a predefined multi-turn question set to assess conversational models across turns for instruction following and dialog coherence, critical capabilities for human-like interaction. Each sequence begins with an initial question, directly followed by a contextual follow-up question. Model responses at each turn are evaluated against human-generated ground truth answers using GPT-4 scoring.
%
%While MTBench comprises eight question categories, we utilized a subset given mobile constraints, differing from conventional benchmarks on PCs and servers. 
%
%Mobile devices have limited memory and slower GPUs, unable to support large models and high precision. LLMs perform poorly on certain tasks like reasoning, math, and coding on mobile devices, yielding meaningless scores low to 1. 
%
Our goal was to tailor benchmarking for mobile insights rather than fully evaluating model capabilities to inspire observations for LLM deployment on mobile devices. We just test two tasks tailored for mobile platforms.
%

\textbf{Task 1} evaluates the extraction ability of an LLM that summarizes a paragraph of text, and \textbf{Task 2} prompts the model to write a paragraph of text.
%
To evaluate model performance on more complex tasks across platforms, a predefined test set was constructed using two challenging extraction and writing tasks from the MTBench multi-turn benchmark dataset.~\footnote{\url{https://huggingface.co/spaces/lmsys/mt-bench}}.
%

Figure~\ref{fig:resource_mtbench} shows the results of memory usage and benchmark scores of two tasks.
%
Profiling showed the GPU operates near saturation with over 95\% utilization on MTBench, while memory increases slightly for multi-turn dialog. 
%
However, the MLC Chat framework does not currently utilize neural processing unit~(NPU) inside mobile SoC, missing optimization evidenced by 0\% utilization of NPU during inference.
%
%

\begin{figure}[ht]
\vspace{-2ex}
\setlength\abovecaptionskip{0pt}
\subfigure[Memory (\%)]{
\includegraphics[width=0.32\textwidth]{figures/eval/mtmempercent.pdf}
\label{fig:mtmem}
}
\hspace{-1.5ex}
\subfigure[Memory (GB)]{
\centering
\includegraphics[width=0.32\textwidth]{figures/eval/mtmem.pdf}
\label{fig:mtmems}
}
\hspace{-1.5ex}
\subfigure[Score]{
\centering
\includegraphics[width=0.32\textwidth]{figures/eval/mtscore.pdf}
\label{fig:mtscores}
}
%\vspace{-1.5ex}
\caption{Memory usage and scores across models~((Llama-2-7B, RedPajama-v1-3B and Vicuna-v1-7B)) and platforms~(IP12-iPhone 12, Pixel 4, S22U-S22 Ultra and Pi-Orange Pi) in MT-Bench evaluation.}
\label{fig:resource_mtbench}
\vspace{-.5ex}
\end{figure}

\textbf{Task 1} and \textbf{Task 2} are more complex than the \textbf{Simple Q\&A} task and are anticipated to use more resources and consume more power. 
%
Figure~\ref{fig:task1_mtbench} and Figure~\ref{fig:task2_mtbench} show the experimental results of power consumption~(mA), throughput~(tok/s) and latency~(s) while running \textit{extraction} and \textit{writing} tasks from MT-Bench test questions.
Results revealed increased energy consumption and latency across all platforms when evaluating models on dialogs with multi-turn questions. 
%
Throughput remained relatively constant for Vicuna-v1-7B, while Llama-2-7B and RedPajama-v1-3B exhibited throughput gains on longer conversations.


\begin{figure}[ht]
\vspace{-2ex}
\setlength\abovecaptionskip{0pt}
\subfigure[Power Consumption]{
\includegraphics[width=0.32\textwidth]{figures/eval/powerTask1.pdf}
\label{fig:task1power}
}
\hspace{-1.5ex}
\subfigure[Throughput]{
\centering
\includegraphics[width=0.32\textwidth]{figures/eval/throughputTask1.pdf}
\label{fig:task1thru}
}
\hspace{-1.5ex}
\subfigure[Latency]{
\centering
\includegraphics[width=0.32\textwidth]{figures/eval/latencyTask1.pdf}
\label{fig:task1latency}
}
%\vspace{-1.5ex}
\caption{\textbf{Task 1 - Extraction} evaluation across models~((Llama-2-7B, RedPajama-v1-3B and Vicuna-v1-7B)) and platforms~(IP12-iPhone 12, Pixel 4, S22U-S22 Ultra and Pi-Orange Pi).}
\label{fig:task1_mtbench}
\vspace{-.5ex}
\end{figure}


\begin{figure}[ht]
\vspace{-2ex}
\setlength\abovecaptionskip{0pt}
\subfigure[Power Consumption]{
\includegraphics[width=0.32\textwidth]{figures/eval/powerTask2.pdf}
\label{fig:task2power}
}
\hspace{-1.5ex}
\subfigure[Throughput]{
\centering
\includegraphics[width=0.32\textwidth]{figures/eval/throughputTask2.pdf}
\label{fig:task2thru}
}
\hspace{-1.5ex}
\subfigure[Latency]{
\centering
\includegraphics[width=0.32\textwidth]{figures/eval/latencyTask2.pdf}
\label{fig:task2latency}
}
%\vspace{-1.5ex}
\caption{\textbf{Task 2 - Writing} evaluation across models~((Llama-2-7B, RedPajama-v1-3B and Vicuna-v1-7B)) and platforms~(IP12-iPhone 12, Pixel 4, S22U-S22 Ultra and Pi-Orange Pi).}
\label{fig:task2_mtbench}
\vspace{-.5ex}
\end{figure}
Figure~\ref{fig:task1_mtbench} and ~\ref{fig:task2_mtbench} indicate that all three models require increased resources, particularly memory, in multi-turn conversation tasks. While resource utilization remains consistent on the iPhone, significant variations are observed across Android platforms. Orange Pi~\cite{OrangePi} runs the model via a command line interface, with less memory utilization.
%

The \textbf{Task2-Writing} exhibited longer latency than \textbf{Task1-extraction}, as text generation produces more words and tokens. Despite increased latency for multi-turn versus simple conversation of \textbf{Simple Q\&A}, RedPajama-v1-3B maintained relatively fast response times for answer generation across tasks.

\vspace{-1ex}
\subsection{Quantization} \label{ssec:quan}
\vspace{-1ex}
We evaluate how various LLM quantization schemes impact resource consumption and user experience on mobile devices, of which observations serve as foundational insights for crafting optimized strategies for LLM deployment on these devices.
%

Quantization can reduce memory and accelerate inference. 
%
MLC~\cite{MLC_LLM} provides options for quantization with quantization 0-bit (q0f16), 3-bit (q3f16), 4-bit (q4f16), and 8bit (q8f16). 
%We compiled the three models with four quantization schemes, including Llama-2-7B, RedPajama-v1-3B, and Vicuna-v1-7B. 
%
Llama-2-7B and Vicuna-v1-7B's resource demands surpassed our testbeds' capacities, particularly in memory. For example, the 8-bit and 0-bit versions of Llama-2-7B need 8.93GB and 15.13GB RAM, whereas iPhone 12 Pro and Pixel 4 offer just 6GB RAM. 
%
Quantization evaluations were performed using the resource-efficient RedPajama-v1-3B model on a Samsung S22 Ultra testbed.

Figure~\ref{fig:usage_quan} illustrates the performance metrics~(latency, memory utilization, and power consumption) of RedPajama-v1-3B under various quantization schemes on the S22 Ultra. Notably, the 3-bit (q3f16) scheme demonstrates decreased memory requirements and quicker inference, benefiting from reduced memory bandwidth and storage needs.
%
In contrast, 0-bit (q0f16) exhibited substantially higher latency and near complete memory usage, representing an infeasible quantization scheme given current mobile device constraints.

\begin{figure}[ht]
\vspace{-2ex}
\setlength\abovecaptionskip{0pt}
\subfigure[Latency]{
\includegraphics[width=0.32\textwidth]{figures/eval/LatencyQuan.pdf}
\label{fig:latency_q}
}
\hspace{-1.5ex}
\subfigure[Memory Usage]{
\centering
\includegraphics[width=0.32\textwidth]{figures/eval/MemQuan.pdf}
\label{fig:thru_q}
}
\hspace{-1.5ex}
\subfigure[Power Consumption]{
\centering
\includegraphics[width=0.32\textwidth]{figures/eval/PowerQuan.pdf}
\label{fig:power_q}
}
%\vspace{-1.5ex}
\caption{Results of evaluation across different quantizations, 0-bit (q0f16), 3-bit (q3f16), 4-bit (q4f16) and 8-bit (q8f16) in latency (s), memory usage and power consumption.}
\label{fig:usage_quan}
\vspace{-.5ex}
\end{figure}


%Although 3-bit (q3f16), 4-bit (q4f16), and 8-bit (q8f16) exhibit relatively lower latency, memory, and energy usage, model performance tradeoffs must also be considered when selecting an appropriate quantization.
%
The precision and answer quality will determine the user experience and quality of the LLM chatbot applications.
We evaluate these four quantization schemes using MT-Bench,
%
as depicted in Table~\ref{tab:scores}.

\begin{table}[htb]
\small
\centering
\caption{The scores of MT-Bench in extraction and writing tasks across various quantization schemes}
\label{tab:scores}
\begin{tabular}{|c|c|c|c|c|}
\hline
                 & 0-bit (q0f16) & 3-bit (q3f16) & 4-bit (q4f16) & 8-bit (q8f16) \\ \hline
Task1-Extraction & 6.4          & 1.4          & 6          & 6          \\ \hline
Task2-Writing    & 7.6          & 3.4          & 6.8          & 7            \\ \hline
\end{tabular}
\end{table}

Results in Table~\ref{tab:scores} show 3-bit quantization provides minor resource savings but falls short of delivering a satisfactory accuracy, while 8-bit incurs overhead without much accuracy gains versus 4-bit. 
%
The 4-bit scheme q4f16 strikes the optimal balance for resource utilization, latency, efficiency, and precision on mobile platforms, achieving a 34.1\% improvement in overall scores compared to 3-bit quantization.

\vspace{-1ex}
\subsection{Model Size} \label{ssec:size}
\vspace{-1ex}
Besides quantization, model size significantly impacts performance and resource utilization. Smaller models with fewer parameters reduce memory requirements and enable faster inference than larger counterparts, which means they are more suitable for devices with limited computational resources.
%
Larger models demand increased resources but can improve performance and provide more precise answers, while smaller models are more efficient yet may sacrifice accuracy.
%
An appropriate tradeoff should be made considering the target platform's capabilities and user requirements.
%
Table~\ref{tab:largemodel} shows RedPajama-1v-7B with extensive parameters has better MTBench scores but higher memory and latency than its smaller counterpart, resulting in reduced throughput. 
%
%
RedPajama-1v-3B yields a slightly reduced MT-Bench score of 6.4 but conserves up to 19.1\% in memory usage.  

%In essence, while larger models may promise improved performance in some scenarios, their demands on memory and computational resources might make them unsuitable for specific applications or devices. Conversely, while smaller models are resource-friendly, there might be challenges regarding their performance or accuracy. The choice between model sizes should be made considering the specific needs and constraints of the intended application.

\begin{table}[htb]
\small
\centering
\caption{The comparison between RedPajama-1v-3B and RedPajama-1v-7B in terms of overall memory usage, latency, and throughput.}
\label{tab:largemodel}
\begin{tabular}{|c|c|c|}
\hline
              & RedPajama-1v-3B & RedPajama-1v-7B \\ \hline
Memory Usage  & 3.86GB          & 5.39GB          \\ \hline
Latency       & 12.3s           & 35.5s           \\ \hline
Throughput & Prefill: 24.8 tok/s Decode: 11.9 tok/s & \multicolumn{1}{l|}{Prefill: 7.84 tok/s Decode: 3.76 tok/s} \\ \hline
MTBench Score & 6.4             & 7.2             \\ \hline
\end{tabular}
\end{table}

\vspace{-1.5ex}
\subsection{Deployment Strategy} \label{ssec:deploy}
\vspace{-1.5ex}
\input{decision}




==> limitations.tex <==
% Limitations (required section)
% Authors are required to discuss the limitations of their work in a dedicated section titled “Limitations”. This section should be included at the end of the paper, before the references, and it will not count toward the page limit. This includes both, long and short papers. Papers without a limitations section will be desk rejected. Note, prior to the December 2023 cycle, this was optional.
\smallskip
\noindent
\textbf{Limitations.}


==> plan.tex <==

https://aclrollingreview.org/cfp#long-papers

